Fixed-Dimensional Energy Games are in Pseudo-Polynomial Time

We generalise the hyperplane separation technique (Chatterjee and Velner, 2013) from multi-dimensional mean-payoff to energy games, and achieve an algorithm for solving the latter whose running time is exponential only in the dimension, but not in the number of vertices of the game graph. This answers an open question whether energy games with arbitrary initial credit can be solved in pseudo-polynomial time for fixed dimensions 3 or larger (Chaloupka, 2013). It also improves the complexity of solving multi-dimensional energy games with given initial credit from non-elementary (Br\'azdil, Jan\v{c}ar, and Ku\v{c}era, 2010) to 2EXPTIME, thus establishing their 2EXPTIME-completeness.

==> proof-arbit.tex <==
\begin{proof}[Proof sketch] We rely for this proof on results proven
  \ifshort\relax\else later \fi in \autoref{sec-fcycle}.  By the
  determinacy of single-cycle bounding games and their equivalence
  with infinite bounding games, it suffices to prove the two `only if'
  directions.

  For~\autoref{th:arbit.1}, assume that Player~1 has a winning strategy
  $\sigma_1$ in the bounding game on $\lossy{V,E,d}$.  In particular,
  there exists a bound $B$ such that Player~1 can maintain
  $\|\rho\|\leq B$ on any play $\rho$ consistent with $\sigma_1$ (an
  explicit such $B$ is provided by \autoref{lem-shp}).  Observe that
  along any consistent play, $\sigma_1$ must always eventually play an
  edge which is not a decrementing self-loop, or the play would
  eventually become unbounded from below.  Hence the following
  strategy $\sigma_1'$ which simply skips all the decrement actions is
  well-defined:
  \begin{equation}
    \sigma_1'(\pi(v,\vec a))\eqdef\begin{cases}
    (v,\vec u,v')&\text{if $\sigma_1(\pi(v,\vec a))=(v,\vec
      u,v')$ with $v\neq v'$}\\&\text{or $\forall 1\leq i\leq d\:.\:\vec u\neq -\vec e_i$},\\
    \sigma_1'(\pi(v,\vec a)(v,\vec a-\vec e_i))&\text{otherwise,
      i.e.\ if there is $1\leq i\leq d$}\\&\text{s.t.\ $\sigma_1(\pi(v,\vec a))=(v,-\vec e_i,v)$.}\end{cases}\end{equation}  By
  monotonicity of energy games, this strategy is winning in the energy
  game on $\tuple{V,E,d}$ with initial credit $B$ on all components.


  %% For the `only if' direction\todo{this is wrong}, assume Player~1 has
  %% a winning strategy $\sigma_1$ in the energy game on $\tuple{V,E,d}$
  %% with initial credit $\vec b$.  Let $B\eqdef\|\vec b\|$; we build a
  %% new strategy $\sigma'_1$ which is winning in the bounding game on
  %% $\lossy{V,E,d}$: it suffices for this to define
  %% \begin{equation}
  %%   \sigma'_1(\pi(v,\vec a))\eqdef\begin{cases}
  %%     (v,-\vec e_i,v)&\text{if $i$ is minimal s.t.\ $\vec a(i)\geq
  %%     B$}\\
  %%     \sigma_1(\pi(v,\vec a))&\text{otherwise, i.e.\ if $\vec
  %%       a(i)<B$ for all $i$.}\end{cases}
  %% \end{equation}
  %% This new strategy contains the play within an hypercube of side
  %% $B+\|E\|$ and Player~1 wins the bounding game.
  %%
  %% For \autoref{th:arbit.1}, let $\vec{b}$ have all entries equal to
  %% the bound in \autoref{th:haupt}, and consider a strategy provided by
  %% that theorem.

  For \autoref{th:arbit.2}, assume that
  Player~2 has a winning strategy in the infinite bounding game on
  $\lossy{V,E,d}$.  Then he has a winning strategy $\sigma_2$
  in the first-cycle bounding game on $\lossy{V,E,D}$, which only plays
  colours that are disjoint from the non-negative orthant
  $\cone{\vec{e}_1, \ldots, \vec{e}_d}$, because
  Player~1 could otherwise use a decrementing self-loop to create a
  cycle outside this colour.  Observe that, for any open half-subspace $H$ 
  that is disjoint from the non-negative orthant, and for any bound $B$,
  there exists a bound on the distances between the boundary of $H$
  and vectors in $H$ whose every component is at least $-B$.
  It follows that the corresponding winning strategy $\widetilde{\sigma_2}$
  of Player~2 in the infinite bounding game (cf.~\autoref{l:Exp})
  is also winning in the energy game $\Delta_{\vec b}\!\tuple{V,E,d}$,
  for all initial credits $\vec b$ (cf.~\autoref{l:unb}).
\end{proof}
% Local IspellDict: british


==> sec-fcycle.tex <==
\subsection{Definition}
Let $G \tuple{V, E, d, \omega}$ denote the following
\emph{first-cycle bounding game}:
\begin{itemize}
\item
at any Player-$1$ vertex, 
Player~$2$ chooses a $|V| \cdot \|\omega\|$-generated
perfect half-space $\ell$ of $\mathbb{Q}^d$,
and then Player~$1$ chooses an outgoing edge,
whose occurence in the play becomes coloured by~$\ell$;
\item
at any Player-$2$ vertex, she chooses an outgoing edge;
\item
the game finishes as soon as a vertex is visited twice,
which produces a simple cycle $C$ with coloured Player-$1$ edges;
\item
Player~$2$ wins if $\omega(C)$, the total weight of the cycle,
is in the largest partially-perfect half-space of $\mathbb{Q}^d$ 
that is contained in all the colours in~$C$;
\item
Player~$1$ wins otherwise.
\end{itemize}

\begin{example}
\label{ex:LR}
In the infinite game on the graph in Fig.~\ref{f:LR},
Player~$1$ can either eventually stay forever at one of the two vertices,
or visit both infinitely often.  In any case, he looses.

Player~$1$ also loses the first-cycle game, from both vertices.
Here $|V| = 2$ and $\|\omega\| = 1$, but the perfect half-spaces
$\ell'_L = \ohsp{\tuple{1, 0}}{\tuple{0, -1}} \,\cup\,
           \ohsp{\vec{0}}{\tuple{-1, 0}}$ and
$\ell'_R = \ohsp{\tuple{1, 0}}{\tuple{0, -1}} \,\cup\,
           \ohsp{\vec{0}}{\tuple{1, 0}}$
are already $1$-generated, where we recall that:
\begin{itemize}
\item
$\ohsp{\tuple{1, 0}}{\tuple{0, -1}}$ is the open half-plane 
$\{\tuple{x, y} \,:\, y < 0\}$;
\item
$\ohsp{\vec{0}}{\tuple{-1, 0}}$ is the open half-line 
$\{\tuple{x, 0} \,:\, x < 0\}$;
\item
$\ohsp{\vec{0}}{\tuple{1, 0}}$ is the open half-line 
$\{\tuple{x, 0} \,:\, x > 0\}$.
\end{itemize}
To win, Player~$2$ chooses $\ell'_L$ at $v_L$, and chooses $\ell'_R$ at $v_R$.
Observe that the largest partially-perfect half-space contained in 
both of the colours is $\ell = \ohsp{\tuple{1, 0}}{\tuple{0, -1}}$,
and the total weight $\tuple{0, -1}$ of the two-vertex cycle is in~$\ell$.
\end{example}

\begin{figure}
\centering
\setlength{\unitlength}{1em}
\begin{tikzpicture}[auto]
\node[rounded corners=.5,regular polygon,regular polygon sides=3,minimum
  size=1cm,draw](L) at (5,2.5){$v_L$};
\node[rounded corners=.5,regular polygon,regular polygon sides=3,minimum
  size=1cm,draw](R) at (13,2.5){$v_R$};
\path[->]
  (L) edge[loop,swap] node{$\tuple{-1, 0}$} ()
  (R) edge[loop,swap] node{$\tuple{1, 0}$} ()
  (L) edge[bend left=15] node{$\tuple{0, -1}$} (R)
  (R) edge[bend left=15] node{$\tuple{0, 0}$} (L);
\end{tikzpicture}
\caption{A $2$-dimensional game graph with only Player-$1$ vertices.}
\label{f:LR}
\end{figure}

\subsection{Transferring Player~$2$'s Strategies}

Suppose $\sigma$ is a strategy of Player~$2$ from a vertex $v_0$
in a first-cycle bounding game $G \tuple{V, E, d, \omega}$.
Let $\widetilde{\sigma}$ be the following strategy of Player~$2$ in
the infinite game $\Gamma \tuple{V, E, d, \omega}$:
\begin{itemize}
\item
at any Player-$2$ vertex, $\widetilde{\sigma}$ chooses 
the edge specified by~$\sigma$;
\item
whenever a cycle is formed, $\widetilde{\sigma}$ cuts it out of its memory,
and continues playing according to~$\sigma$.
\end{itemize}

\begin{lemma}
\label{l:Exp}
If $\sigma$ is winning in $G \tuple{V, E, d, \omega}$,
then $\widetilde{\sigma}$ is winning in $\Gamma \tuple{V, E, d, \omega}$.
\end{lemma}

\begin{proof}
Consider any infinite play $\rho$ of $\widetilde{\sigma}$, and let:
\begin{itemize}
\item
$\rho^\sharp$ be obtained from $\rho$ by colouring all Player~$1$'s edges with 
the $|V| \cdot \|\omega\|$-generated perfect half-spaces of $\mathbb{Q}^d$
as specified by~$\sigma$;
\item
$C_1, C_2, \ldots$ be the cycle decomposition of~$\rho^\sharp$;
\item
$\ell_i$ be the largest partially-perfect half-space of $\mathbb{Q}^d$
that is contained in all the colours in $C_i$, for each~$i$.
\end{itemize}
The rest is an exercise for the reader.
(\emph{Hint:}\/ First show that, for any $i$, 
either $\ell_i$ contains $\ell_{i + 1}$ or vice-versa.
Infer that the set of all $|V| \cdot \|\omega\|$-generated 
partially-perfect half-spaces of $\mathbb{Q}^d$ that 
occur infinitely often in the sequence $\ell_1, \ell_2, \ldots$ 
has an element that is contained in all the others.  
Then apply Lem.~\ref{l:unb}.)
\qed
\end{proof}


\subsection{Transferring Player~$1$'s Winning Strategies}

For any $k$-dimensional open half-space $H$ in $\mathbb{Q}^d$, let:
\begin{itemize}
\item
$\overline{H}$ denote the $k$-dimensional closure of~$H$;
\item
$\widehat{H} = \vsp{H} \setminus \overline{H}$ denote 
the open-half space dual to~$H$.
\end{itemize}

Suppose $\sigma$ is a strategy of Player~$1$ from a vertex $v_0$
in a first-cycle bounding game $G \tuple{V, E, d, \omega}$,
which is winning.  We now define a strategy $\widetilde{\sigma}$ 
of Player~$1$ in the infinite game $\Gamma \tuple{V, E, d, \omega}$.

The memory of $\widetilde{\sigma}$ consists of:
\begin{itemize}
\item
a simple path $\gamma$ from the initial vertex $v_0$ to the current vertex~$v$,
in which Player~$1$'s edges are coloured by $|V| \cdot \|\omega\|$-generated
perfect half-spaces of~$\mathbb{Q}^d$;
\item
a $|V| \cdot \|\omega\|$-generated perfect half-space $\ell$ of~$\mathbb{Q}^d$;
\item
for each $k \in \{d, \ldots, 1, 0\}$ 
and each nonzero total weight $W$ of a simple cycle,
a natural number $\mathsf{c}(k, W)$.
\end{itemize}
Initially, $\ell$ is the $\prec$-minimal colour
and all counters $\mathsf{c}(k, W)$ have value~$0$.

At any Player-$1$ vertex, $\widetilde{\sigma}$ chooses the edge that
$\sigma$ specifies for history $\gamma$ and colour $\ell$.
After any move that leads to a vertex not occuring in $\gamma$,
the memory of $\widetilde{\sigma}$ is updated only by extending $\gamma$.
Otherwise, a cycle $C$ is formed, and the memory is updated as follows:
\begin{itemize}
\item
$C$ is cut out of~$\gamma$.
\item
Counter $\mathsf{c}(0, \omega(C))$ is incremented,
unless $\omega(C) = \vec{0}$.
If, for all $k \in \{d, \ldots, 1\}$ and all simple-cycle weights 
$W \in \widehat{\ell(k)}$, we have
\begin{equation}
\tsum_{j = 0}^k \mathsf{c}(j, W) <
(4 |V| \cdot \|\omega\|)^{2 k (d + 2)^2},
\tag{$*$}
\end{equation}
then the memory update is finished.
If not, let $k \in \{d, \ldots, 1\}$ be the largest for which 
the inequality ($*$) fails for some $W \in \widehat{\ell(k)}$.
By Prop.~\ref{pr:ssw}, Lem.~\ref{l:alt} and Lem.~\ref{l:small}, 
there are two cases:
  \begin{itemize}
  \item[($\dag$)]
  \emph{There exists a $|V| \cdot \|\omega\|$-generated open half-space $H$
        of $\vsp{\ell(k)}$ such that ($*$) holds for all
        simple-cycle weights $W \in \widehat{H}$.}
  In this case, $\ell$ is replaced by $\ell^\gg_H$,
  for the $<$-minimal such $H$.
  The following updates are performed in parallel,
  for all $W$ and all $k' \in \{k - 1, \ldots, 0\}$:
  \begin{align*}
  \mathsf{c}(k, W)  & := \tsum_{j = 0}^k \mathsf{c}(j, W) &
  \mathsf{c}(k', W) & := 0
  \end{align*}
  \item[($\ddag$)]
  \emph{$A \vec{x} = \vec{0}$, where the columns of matrix $A$ are
        an enumeration $W_1, \ldots, W_n$ of all nonzero simple-cycle weights
        in $\vsp{\ell(k)}$ that fail ($*$), has a solution in positive integers
        bounded by $(2 (|V| \cdot \|\omega\| + 1))^{(k + 2)^2}$.}
  Here, $\ell$ is replaced by $\ell^\gg_{H^\sharp}$,
  for the $<$-minimal $|V| \cdot \|\omega\|$-generated
  open half-space $H^\sharp$ of $\vsp{\ell(k)}$.
  Provided $\lambda$ is a positive integer such that, for all~$W_i$,
  \begin{equation}
  0 \leq \tsum_{j = 0}^k \mathsf{c}(j, W_i) - \lambda \cdot \vec{x}(i) <
         (4 |V| \cdot \|\omega\|)^{2 k (d + 2)^2},
  \tag{$**$}
  \end{equation}
  the following updates are performed in parallel,
  for all $W_i$, all other simple-cycle weights $W'$
  and all $k' \in \{k - 1, \ldots, 0\}$:
  \begin{align*}
  \mathsf{c}(k, W_i)  & := \tsum_{j = 0}^k \mathsf{c}(j, W_i) -
                           \lambda \cdot \vec{x}(i)          &
  \mathsf{c}(k', W_i) & := 0                                 \\
  \mathsf{c}(k, W')   & := \tsum_{j = 0}^k \mathsf{c}(j, W') &
  \mathsf{c}(k', W')  & := 0
  \end{align*}
  If no such $\lambda$ exists, the $k^{\text{th}}$ alarm button is pressed.
  \end{itemize}
\end{itemize}

Let us indicate that an occurence of case ($\dag$) or case ($\ddag$)
is with a particular value of $k$ by calling it \emph{$k$-level}.
In any play of $\widetilde{\sigma}$,%
\footnote{The following notions require that 
either annotated plays are considered,
or the choice between ($\dag$) and ($\ddag$) when both are possible,
as well as the choices of $\vec{x}$ and $\lambda$ in case ($\ddag$), 
are made deterministic.}
let us say that:
\begin{itemize}
\item
a \emph{$k$-month} is any maximal segment in which 
every occurence of case ($\dag$) is $< k$-level and 
every occurence of case ($\ddag$) is $< k$-level;
\item
a \emph{$k$-year} is any maximal segment in which 
every occurence of case ($\dag$) is $\leq k$-level and 
every occurence of case ($\ddag$) is $< k$-level.
\end{itemize}

\begin{lemma}
\label{l:Bnd}
\begin{enumerate}
\item\label{l:Bnd.1}
Any $(k + 1)$-month is a sequence of $k$-years,
and any $k$-year is a sequence of $k$-months.
\item\label{l:Bnd.2}
During any $k$-month, 
all the colours contain the same $k$-perfect half-space,
and the counters $\mathsf{c}(k', W)$ with $k' \geq k$ do not change.
\item\label{l:Bnd.3}
During any $k$-year,
the colour's $k$-dimensional component open half-space
increases with respect to the $<$ ordering whenever the $k$-month changes,
and the counters $\mathsf{c}(k, W)$ never decrease.
\item\label{l:Bnd.4}
Before the parallel update of the counters at the end of any $k$-month, 
letting $H$ be the $k$-dimensional component open half-space
of the $k$-month's colours, we have that:
  \begin{itemize}
  \item
  $\tsum_{j = 0}^{k - 1} \mathsf{c}(j, W) < |V|$
  for all $W$ in~$H$;
  \item
  if $k \geq 2$, then
  $\tsum_{j = 0}^{k - 1} \mathsf{c}(j, W) <
   2 (4 |V| \cdot \|\omega\|)^{2 (k - 1) (d + 2)^2}$
  for all $W$ in the boundary of~$H$.
  \end{itemize}
\item\label{l:Bnd.5}
Before the parallel update of the counters at the end of any $k$-year, we have
\[\tsum_{j = 0}^k \mathsf{c}(j, W) <
  2 (4 |V| \cdot \|\omega\|)^{2 k (d + 2)^2}\]
for all $W$ in the $k$-dimensional component subspace 
of the $k$-year's colours.
\item\label{l:Bnd.6}
For all $k$, the $k^{\text{th}}$ alarm button is never pressed.
\item\label{l:Bnd.7}
The total weight of the play so far always equals
the total weight of the simple path $\omega(\gamma)$ plus
the weighted sum of all the counters 
$\tsum_{j = 0}^d \tsum_W \mathsf{c}(j, W) \cdot W$.
\item\label{l:Bnd.8}
Strategy $\widetilde{\sigma}$ is winning in $\Gamma \tuple{V, E, d, \omega}$.
\end{enumerate}
\end{lemma}

\begin{proof}
Parts \ref{l:Bnd.1}, \ref{l:Bnd.2} and \ref{l:Bnd.3} are straightforward.

We establish parts \ref{l:Bnd.4}, \ref{l:Bnd.5} and \ref{l:Bnd.6} together.

For the first half of part~\ref{l:Bnd.4}, observe that, 
during the $k$-month, strategy $\widetilde{\sigma}$ chooses the edges 
specified by strategy $\sigma$ for the $k$-month's colours, 
and that for any nonempty subset $L$ of those colours, 
the greatest partially-perfect half-space that is 
contained in all members of $L$ necessarily contains $H$.
Recalling that $\sigma$ is winning for Player~$1$ in the first-cycle game, 
it follows that cycles whose weight is in $H$ can only be formed 
by consuming edges that were in the simple path $\gamma$ 
at the beginning of the $1$-month.

We have the second half of part~\ref{l:Bnd.4} by part~\ref{l:Bnd.5} for $k - 1$.

For parts \ref{l:Bnd.5} and \ref{l:Bnd.6}, 
we rely on part~\ref{l:Bnd.4} for the same $k$.
Since the $k$-year is either the initial one, 
or it begins with a $k$-level occurence of case ($\ddag$) which is successful 
(i.e., in which the $k^{\text{th}}$ alarm button is not pressed),
or it begins with a $> k$-level occurence of ($\dag$) or ($\ddag$),
we have that, at the beginning of the $k$-year, 
the inequality ($*$) holds for all $W$ in the $k$-dimensional subspace $S$.
Observe that, for any such $W$, the inequality ($*$) 
continues to hold until a suffix (possibly empty) of the sequence of 
$k$-months that makes up the $k$-year, and during the latter, 
$W$ is always in the closed half-space $\overline{\ell(k)}$.
Using part~\ref{l:Bnd.4} and Prop.~\ref{pr:sib}, we infer for all $W$ in $S$,
that before the parallel update of the counters at the end of the $k$-year,
if $k = 1$ then
\begin{multline*}
\tsum_{j = 0}^k \mathsf{c}(j, W) -
(4 |V| \cdot \|\omega\|)^{2 k (d + 2)^2} < \\
2 (2 |V| \cdot \|\omega\| + 1)^{d (k - 1)} \cdot |V| \leq 
(4 |V| \cdot \|\omega\|)^{(2 k - 1) (d + 2)^2},
\end{multline*}
and for $k \geq 2$ we have
\begin{multline*}
\tsum_{j = 0}^k \mathsf{c}(j, W) - 
(4 |V| \cdot \|\omega\|)^{2 k (d + 2)^2} < \\
2 (2 |V| \cdot \|\omega\| + 1)^{d (k - 1)} \cdot 
2 (4 |V| \cdot \|\omega\|)^{2 (k - 1) (d + 2)^2} \leq 
(4 |V| \cdot \|\omega\|)^{(2 k - 1) (d + 2)^2}.
\end{multline*}
The inequality asserted in part~\ref{l:Bnd.5} follows because 
$2 k - 1 \leq 2 k$.
Moreover, if the $k$-year ends with a $k$-level occurence of case ($\ddag$), 
the $k^{\text{th}}$ alarm button is not pressed since
\begin{multline*}
(4 |V| \cdot \|\omega\|)^{(2 k - 1) (d + 2)^2} \cdot
(2 (|V| \cdot \|\omega\| + 1))^{(k + 2)^2} \leq \\
(4 |V| \cdot \|\omega\|)^{(2 k - 1) (d + 2)^2} \cdot
(4 |V| \cdot \|\omega\|)^{(d + 2)^2} = 
(4 |V| \cdot \|\omega\|)^{2 k (d + 2)^2},
\end{multline*}
which is the bound in the inequality~($*$).

Part~\ref{l:Bnd.7} is straightforward.

Part~\ref{l:Bnd.8} follows from the preceding parts, which give us that, 
for all $W$ we have always:
\[\tsum_{j = 0}^d \mathsf{c}(j, W) < 
  2 (4 |V| \cdot \|\omega\|)^{2 d (d + 2)^2}.
  \qedmath\]
\end{proof}


\subsection{The Hauptsatz}

Putting Lem.~\ref{l:Exp} and Lem.~\ref{l:Bnd} together,
and observing that
\[(|V| - 1) \cdot \|\omega\| + 
  2 (4 |V| \cdot \|\omega\|)^{2 d (d + 2)^2}
    \cdot |V| \cdot \|\omega\| \leq
  (4 |V| \cdot \|\omega\|)^{2 (d + 2)^3},\]
we obtain our main result on the first-cycle and infinite bounding games:

\begin{theorem}
\label{th:haupt}
From any vertex in any multi-weighted game graph $\tuple{V, E, d, \omega}$,
either Player~$1$ or Player~$2$ wins 
both the first-cycle game $G \tuple{V, E, d, \omega}$ 
and the infinite game $\Gamma \tuple{V, E, d, \omega}$.
Also, for any winning strategy $\sigma$ in $G \tuple{V, E, d, \omega}$,
the strategy $\widetilde{\sigma}$ we defined is winning in 
$\Gamma \tuple{V, E, d, \omega}$, and in the case of Player~$1$,
it ensures that the norms of the total weights of all finite plays
are at most $(4 |V| \cdot \|\omega\|)^{2 (d + 2)^3}$.
\end{theorem}

% Local IspellDict: british


==> sec-pseudo-bases.tex <==
Throughout this section, we work in rational spaces.

\subsubsection{Pseudo-Independence and Pseudo-Bases}  Fix some finite
set of integer vectors $\vec V\subseteq\+Z^d$ for some dimension $d$.
A subset $\{\vec v_1,\dots,\vec v_m\}$ of $\vec V$ is
\emph{pseudo-dependent} if there exist $x_1,\dots,x_m$ in $\+N$ not
all zeroes such that
\begin{equation}\label{eq-pseudo-dep}
  \sum_{i=1}^m x_i\vec v_i = 0\;.
\end{equation}
Note that we could also define pseudo-dependence with $x_1,\dots,x_m$
non-negative rationals in $\+Q_{\geq 0}$ instead of $\+N$ to the same
effect.

A subset $\{\vec v_1,\dots,\vec v_m\}$ of $\vec V$ where the only
solution to \eqref{eq-pseudo-dep} is the trivial solution
$x_1=\cdots=x_m=0$ is called accordingly a \emph{pseudo-independent}
set.  %   Equivalently, \todo{This is just for the insight, I never use it
%   later.} a subset $\{\vec v_1,\dots,\vec v_m\}$ of $\vec V$ is
% pseudo-independent if and only if its \emph{convex hull}
% \begin{equation}\label{eq-conv-hull}
%   \mathrm{Hull}(\{\vec v_1,\dots,\vec v_m\})\eqdef\left\{\sum_{i=1}^{m}y_i\vec
% v_i\mathrel{\Bigg|}\sum_{i=1}^my_i=1\wedge\forall 1\leq i\leq
% m.y_i\in\+R_{\geq 0}\right\}
% \end{equation}
% does not contain the null vector $\vec 0$.
% 
A \emph{pseudo-basis} of $\vec V$ is then a pseudo-independent subset
of $\vec V$ maximal for inclusion.  Pseudo-bases are somewhat
degenerate bases: they must include some basis of $\vec V$, possibly
in addition to some dependent vectors:
\begin{lemma}\label{lem-pb-dim}
  If $\vec B$ is a pseudo-basis of $\vec V$, then $\mathrm{dim}(\vec
  B)=\mathrm{dim}(\vec V)$.
\end{lemma}
\begin{proof}
  Let $\vec B=\{\vec v_1,\dots,\vec v_m\}$ be a pseudo-independent
  subset of $\vec V$ of dimension $\ell<\mathrm{dim}(\vec V)$.
  Up to reordering, we assume $\{\vec v_1,\dots,\vec v_\ell\}$ to be a
  basis of $\vec B$, i.e.\ any vector $\vec v_j$ for $\ell+1\leq j\leq
  m$ can be expressed as a linear combination of the $\vec v_i$ for
  $1\leq i\leq \ell$.  We are going to show that $\vec B$ is not a
  pseudo-basis of $\vec V$.

  Since $\ell<\mathrm{dim}(\vec V)$, there exists a vector $\vec v_0$
  in $\vec V\setminus \vec B$ such that $\{\vec v_0,\dots,\vec
  v_\ell\}$ is independent---otherwise $\vec V$ would be of dimension
  $\ell$.  Consider $\vec B'\eqdef\vec B\uplus\{\vec v_0\}$.  Assume
  $\vec B'$ is pseudo-dependent, i.e.\ assume that there exist
  $x_0,\dots,x_m$ in $\+N$ not all zeroes such that $\sum_{i=0}^\ell
  x_i\vec v_i+\sum_{j=\ell+1}^mx_j\vec v_j=0$.  Because each $x_j\vec
  v_j$ can be expressed as a linear combination of the $\vec v_i$ for
  $1\leq i\leq \ell$, this contradicts $\{\vec v_0,\vec v_1,\dots,\vec
  v_\ell\}$ being independent.  Thus $\vec B'$ must be
  pseudo-independent, and $\vec B$ cannot be maximal.
\end{proof}

\subsubsection{Salient Cones}
A natural geometric counterpart to pseudo-independent sets $\{\vec
v_1,\dots,\vec v_m\}$ are \emph{salient cones}: any set $\{\vec
v_1,\dots,\vec v_m\}$ defines a \emph{cone} by
\begin{equation}
  \mathrm{Cone}(\{\vec v_1,\dots,\vec v_m\})\eqdef\left\{\sum_{i=1}^{m}z_i\vec
    v_i\mathrel{\Bigg|}\forall 1\leq i\leq m.z_i\in\+Q_{\geq 0}\right\}\;.
\end{equation}
Observe that the cones associated with pseudo-independent sets are
necessarily \emph{salient}, in that the only vector $\vec v$ in the
cone such that $-\vec v$ is also in the cone is $\vec v=\vec 0$.
Conversely, if a set $\{\vec v_1,\dots,\vec v_m\}$ defines a salient
cone and $\vec v_i\neq\vec 0$ for all $1\leq i\leq m$, then the only
solution to \eqref{eq-pseudo-dep} is the trivial one.
Thus pseudo-bases can also be seen as maximal subsets of $\vec
V\setminus\{\vec 0\}$ generating salient cones.

\begin{lemma}\label{lem-pb-cones}
  Let $\vec B$ be a pseudo-basis of $\vec V$ and $\vec v_0$ be a
  vector in $\vec V$.  Then either $\vec v_0$ is in $\vec B$ or
  $-\vec v_0$ is in $\mathrm{Cone}(\vec B)$.
\end{lemma}
\begin{proof}
  Let $\vec B=\{\vec v_1,\dots,\vec v_m\}$ be a pseudo-basis of $\vec
  V$.  If $\vec v_0$ is a vector in $\vec V\setminus \vec B$, then by
  maximality of $\vec B$ there exists a non-trivial non-negative
  integer solution to $\sum_{i=0}^m x_i\vec v_i=0$, i.e.\ $-\vec v_0$
  belongs to $\mathrm{Cone}(\vec B)$.  Conversely, if $-\vec v_0$
  is in $\mathrm{Cone}(\vec B)$, since the latter is salient, then
  $\vec v_0$ is not in $\mathrm{Cone}(\vec B)$, and thus not in
  $\vec B$.
\end{proof}

\subsubsection{Counting Pseudo-Bases}
Our goal in the remainder of this section is to bound the number of
pseudo-bases of $\vec V$ given $r\eqdef \mathrm{dim}(\vec V)\leq d$
the dimension of the vector space generated by $\vec V$ and $n\eqdef
|\vec V|$ the cardinality of $\vec V$.  More precisely, we would like
a polynomial bound in $n$ when $d$ (and thus $r$) is fixed; see the
statement of \autoref{th-pb}.
\begin{example}[Pseudo-bases over the line]\label{ex-pbline}
  Assume $d=1$, i.e.\ $\vec V$ is a set of integers.  Then there are
  at most two pseudo-bases, namely $\vec V_{<0}\eqdef\{\vec v\in\vec
  V\mid \vec v<0\}$ and $\vec V_{>0}\eqdef\{\vec v\in\vec V\mid \vec
  v>0\}$ when they are non-empty.
\end{example}
\begin{example}[Pseudo-bases of an independent set]
  Assume $r=n$, i.e.\ that $\vec V$ is an independent set.  Because
  any independent set is also pseudo-independent, $\vec V$ is its own
  sole pseudo-basis.
\end{example}
% \noindent \autoref{ex-pbline} shows that $\vec V\setminus\vec B$ can
% contain another pseudo-basis.

\begin{theorem}\label{th-pb}
  Let $\vec V$ be a finite subset of $\+Z^d$ for some $d$.  Then there
  are at most $O(|\vec V|^{d-1})$ pseudo-bases of $\vec V$.
\end{theorem}
\begin{proof}
  The main intuition behind our bound on the number of pseudo-bases is
  to consider the \emph{faces} of their generated cones.  Let $\vec F$
  be an independent subset of $\vec V$ of dimension $r-1$, thus
  spanning a hyperplane $H_{\vec F}$ passing through the origin.  If
  $\vec B$ is a pseudo-basis of $\vec V$ containing $\vec F$, we say
  that $\vec F$ \emph{supports} $\vec B$ if
  \begin{enumerate}
  \item\label{support-1} $H_{\vec F}\cap\mathrm{Cone}(\vec
    B)=\mathrm{Cone}(\vec F)$, and
  \item\label{support-2} $H_{\vec F}$ splits the vector space
    generated by $\vec V$ into two closed linear half-spaces, one of
    which contains $\vec B$, i.e.\ if $H_{\vec F}$ can be written as
    $\{\vec x\mid\vec c\vec x=0\}$ with $\vec c\vec v\geq 0$ for all
    $\vec v\in\vec B$.
  \end{enumerate}

  By \autoref{cl-pb-1} below, each $r-1$ tuple of independent vectors
  in $\vec V$ can be the support of at most two pseudo-bases of $\vec
  V$.  There are therefore at most $2\binom{n}{r-1}$ pseudo-bases of
  $\vec V$, which proves the theorem.
  
  \begin{claim}\label{cl-pb-1}
    An independent subset $\vec F\subseteq\vec V$ of dimension $r-1$
    supports at most two different pseudo-bases of $\vec V$.
  \end{claim}
  In order to prove \autoref{cl-pb-1}, assume for the sake of
  contradiction that $\vec F=\{vec v_1,\dots,\vec v_{r-1}\}$ supports more
  than two pseudo-bases of $\vec V$, and let $H_{\vec F}$ be its
  spanned hyperplane.  Then $H_{\vec F}=\{\vec x\mid\vec c\vec x=0\}$
  splits the space into two linear half-spaces, and by
  \eqref{support-2} one of these two half-spaces must contain at least
  two different pseudo-bases $\vec B$ and $\vec B'$ of $\vec V$, i.e.\
  $\vec c\vec v\geq 0$ for all $\vec v\in\vec B\cup\vec B'$.  In fact,
  this yields that $\vec c\vec v\geq0$ for all $\vec v$ in
  $\mathrm{Cone}(\vec B)$ or $\mathrm{Cone}(\vec B')$.

  Because both $\vec B$ and $\vec B'$ are maximal pseudo-independent
  sets, none is included in the other.  Consider some vector $\vec
  v_0$ in $\vec B'\setminus\vec B$.  By \autoref{lem-pb-cones}, $-\vec
  v_0$ is in $\mathrm{Cone}(\vec B)$, hence $\vec c\vec v_0\leq 0$ and
  $\vec v_0$ is in the \emph{other} linear half-space defined by
  $H_{\vec F}$.  Thus $\vec v_0$ must be contained in $H_{\vec F}$
  itself, i.e.\ $\vec c\vec v_0=0$, or we would have a contradiction
  with the hypothesis $\vec v_0\in\vec B'$.
 
  In order to derive a contradiction in this last case, we show next
  that $\{\vec v_0\}\uplus\vec B$ is pseudo-independent, which
  contradicts the maximality of $\vec B$ and concludes the proof:
  By~\eqref{support-1} and since $\vec v_0$ is in $H_{\vec
    F}\cap\mathrm{Cone}(\vec B')$, it is in $\mathrm{Cone}(\vec F)$,
  i.e.\ there exist $z_1,\dots,z_{r-1}\geq 0$ such that
  \begin{equation}\label{eq-cl-pb-1}
    \vec v_0=\sum_{i=1}^{r-1}z_i\vec v_i\;.
  \end{equation}
  Note that the $z_i$'s cannot be all zeroes, or $\vec v_0$ would be
  equal to $\vec 0$ and $\vec B'$ would not be pseudo-independent.

  Assume now that $\{\vec v_0\}\uplus\vec B$ is pseudo-dependent,
  i.e.\ that there exist $x_0,\dots,x_m\geq 0$ not all zeroes such
  that
  \begin{align}
    x_0\vec v_0+\sum_{i=1}^{r-1}x_i\vec v_i+\sum_{j=r}^mx_j\vec
    v_j&=0\;.
    \intertext{By \eqref{eq-cl-pb-1}, this yields}
    \sum_{i=1}^{r-1}(x_i+x_0z_i)\vec v_i+\sum_{j=r}^mx_j\vec
    v_j&=0\;.
  \end{align}
  Because $\vec B$ is pseudo-independent and all the coefficients are
  non-negative, this entails that
  \begin{itemize}
    \item $x_j=0$ for all $r\leq j\leq m$, and
    \item $x_i+x_0z_i=0$ for all $1\leq i\leq r-1$.
  \end{itemize}
  Thus either $x_0=0$ and $x_i=0$ for all $0\leq i\leq m$, or $x_0>0$
  and $z_i=0$ for all $1\leq i\leq r-1$, both contradicting our
  hypotheses on the coefficients $z_i$ and $x_i$.
\end{proof}

\todo{I could illustrate the case $d=r=2$ with a figure here.}
% Local IspellDict: british

